Additive Multi-Index Gaussian process modeling, with application to multi-physics surrogate modeling of the quark-gluon plasma

The Quark-Gluon Plasma (QGP) is a unique phase of nuclear matter, theorized to have filled the Universe shortly after the Big Bang. A critical challenge in studying the QGP is that, to reconcile experimental observables with theoretical parameters, one requires many simulation runs of a complex physics model over a high-dimensional parameter space. Each run is computationally very expensive, requiring thousands of CPU hours, thus limiting physicists to only several hundred runs. Given limited training data for high-dimensional prediction, existing surrogate models often yield poor predictions with high predictive uncertainties, leading to imprecise scientific findings. To address this, we propose a new Additive Multi-Index Gaussian process (AdMIn-GP) model, which leverages a flexible additive structure on low-dimensional embeddings of the parameter space. This is guided by prior scientific knowledge that the QGP is dominated by multiple distinct physical phenomena (i.e., multiphysics), each involving a small number of latent parameters. The AdMIn-GP models for such embedded structures within a flexible Bayesian nonparametric framework, which facilitates efficient model fitting via a carefully constructed variational inference approach with inducing points. We show the effectiveness of the AdMIn-GP via a suite of numerical experiments and our QGP application, where we demonstrate considerably improved surrogate modeling performance over existing models.

==> trash.tex <==
\section{Numerical Illustration}
\label{sec:exp}
We now demonstrate the functionality of our additive specification for modeling more complex underlying functions defined on varying dimensions and sample sizes. We will also compare our method to the full suite of the state of the art. Consider the following synthetic function that composed of 3 additive functions that each vary along their own separate $2$-d linear embeddings. 

\begin{align*}
    &y_i = .5f(\bm{u}^i) + .3g(\bm{v}^i) + .2h(\bm{k}^i) + \epsilon_i \ , \ \bm{u}^i, \bm{v}^i, \bm{k}^{i} \in \mathbb{R}^2 \\
    &f(\bm{u}_i) = sin(1.25\bm{u}^i_0) + cos(.5\bm{u}^i_1) \ , \  \bm{u}^i = M_1\bm{x}^i \ , \ \bm{x}^i \sim \w{MVN}(0_{Dx1}, I_{DxD})  \\
    &g(\bm{v}_i) = cos(.5\bm{v}^i_0\bm{v}^i_1)\ , \
    \bm{v}^i = M_2\bm{x}^i \\
    &h(\bm{k}_i) = \bm{k}^i_1cos(.5\bm{k}^i_0)\ , \
    \bm{k}^i = M_3\bm{x}^i \\ 
    &\bm{x}^i \sim \w{MVN}(0_{Dx1}, I_{DxD})
\end{align*}
 $M_1, M_2, M_3 \in \mathbb{R}^{2xD}$ embed the D dimensional input observations into three distinct $2$-d linear sub-spaces. We generate each $M_l$ by drawing $M'_l \sim \w{MN}(0, I_{2x2}, I_{DxD})$ and then normalizing to obtain $M_l =\frac{M'_l}{sd(vec(M_l'\bm{X}^T))}$. This normalization ensures that the random lower dimensional embedding maps input points into a consistently sized and positioned region of $\mathbb{R}^2$ across simulations. We set $\sigma$ to be 15\% of the standard deviation of the random variable $.5f(\bm{u}^i) + .3g(\bm{v}^i) + .2*h(\bm{k}^i)$. We estimate this standard deviation using monte-carlo. 
 
 We use the process above to generate sample ten data sets with varying training sample sizes. We will examine performance of models using data sets of sizes $n = 300, 400, 500$ and original dimension $D = 20, 25, 30$ We generate 10 data sets for each combinations settings and will evaluate the predictive performance on $300$ testing data points. 
 
 We first compare the performance of vanilla ARD-GP with AdMIn-GP using 1 and 3 additive components. We also compare to DLE-GP and DPA-GP methods. We specify the dimension of the linear embeddings of our 3 additive component model to be 5. We set the DLE-GP, DPA-GP and single component AdEm-GP embedding dimensions to be $d = 15$ so that every method can utilize the same number of features/dimension. The results do not change significantly for other choices of $d$. 
 
 \cmtS{should still include the results of this model (Gramacy's Bayesian version?) given a reasonable running time / \# of MCMC runs.}
 
We see in Figure \ref{fig:mixexp} that the 1 and 3 component AdEm-GP model out-perform the other methods  across sample sizes and original data dimension for all metrics. AdEm-GP 3 performance improves relative to AdEm-GP 1 as the sample size increases. In addition, the ELBO successfully chose the number of additive-components with the lower RMSE/CRPS in every trial. We see that DLE-GP and DPA-GP exhibit very unstable behavior due to the difficulty of optimizing a large number of parameters using relatively few data points and no shrinkage \citep{snelson_variable_2012}. In addition, only the AdEm-GP models achieve consistent 95\% coverage for all sample sizes. Ultimately, AdEM-GP combined with ELBO model selection for the additive components provides the best prediction and uncertainty quantification.

We next examine fitting different numbers of additive mixtures to the data. Figure \ref{fig:mix_comp} shows the predictive results of fitting the 1, 2,3, and 4 additive component models  We define the linear embedding dimensions for each model's component's as 15, 8, 5, and 4 respectively so that model has access to a similar number of features. The first 2 columns of \ref{fig:mix_comp} show that the model is generally robust to mis-specification with the multi-component models all performing fairly well relative to the single component model. However, as the sample size and dimension increases, we see that the 3 mixture model out performs the other component models. 

We also note that the ELBO performs effective model selection for the number of components.The last column of \ref{fig:mix_comp} also shows the ELBO of each fit subtracted by the ELBO for the AdEM-GP 3 and divided by sample size. We see that for higher sample sizes and dimensions, all other models have negative ELBO relative to the ground truth 3-component model. For smaller sample sizes and dimensions, the ELBO is  more ambivalent between models which reflects the similarity of the model's predictive results. 

 \cmtS{May need a few more experiments:
 \begin{itemize}
 \item How does our model work under misspecifications on rank / mixtures? also (with true mixtures = 3), see how model performs with specified mixture = 5 (we have mixture = 1)?
 \item Might also be worth exploring effect of dimensionality - this would be a strong case for our model. E.g., use the above base case, then increase dimensionality to 20, 25 (then use 15 as a base case)? Also explore what happens when the true rank = 4? What recommendations would we make on sample size rule of thumb? (leave this here for now - I might write something later on.)
 \end{itemize}
 }
 
 


\begin{figure}[h]
\centering
\includegraphics[width = \textwidth]{figs/other_mix.png}
\caption{Predictive metrics for GP methods applied to synthetic mixture example across sample sizes}
\label{fig:mixexp}
\end{figure}


\begin{figure}[h]
\centering
\includegraphics[width = \textwidth]{figs/mix_mix.png}
\caption{Comparison between different numbers of additive components in the AdMIn-GP Model. Row represent different dimensionality of the original data.}
\label{fig:mix_comp}
\end{figure}


